Learning Coarse-Grained Dynamics on Graph

We consider a Graph Neural Network (GNN) non-Markovian modeling framework to identify coarse-grained dynamical systems on graphs. Our main idea is to systematically determine the GNN architecture by inspecting how the leading term of the Mori-Zwanzig memory term depends on the coarse-grained interaction coefficients that encode the graph topology. Based on this analysis, we found that the appropriate GNN architecture that will account for $K$-hop dynamical interactions has to employ a Message Passing (MP) mechanism with at least $2K$ steps. We also deduce that the memory length required for an accurate closure model decreases as a function of the interaction strength under the assumption that the interaction strength exhibits a power law that decays as a function of the hop distance. Supporting numerical demonstrations on two examples, a heterogeneous Kuramoto oscillator model and a power system, suggest that the proposed GNN architecture can predict the coarse-grained dynamics under fixed and time-varying graph topologies.

==> _arc/_dyn.tex <==
% ----------------------------------
\section{Dynamics on Graphs}
% ----------------------------------
In this section, we provide the notations for dynamics on graphs and discuss two relevant examples that will be numerically investigated in this paper. 


We first define the graph structure that may have time-varying topology.  At time $t$, let $\cG_t=(\cV,\cE_t,\cW_t)$ be a graph with a set of $N$ nodes, $\cV\subset\bN^+$, a set of edges $\cE_t\subseteq\cV\times\cV$, and the edge weights $\cW_t=\{w_{ij,t}|w_{ij,t}\in\bR,(i,j)\in\cE_t,t\in\bR^+\}$.  The graph may contain self-connections, e.g., for node $i$, $(i,i)\in\cE_t$.  The graph may contain directed connections between nodes $i$ and $j$, which entails two cases: (1) $(i,j)\in\cE_t$ and $(j,i)\notin\cE_t$, or (2) $\{(i,j),(j,i)\}\subset\cE_t$ and $w_{ij,t}\neq w_{ji,t}$.
For node $i$, define its 0-hop neighbor as itself $\cN_i^{(0)}=\{i\}$, and its 1-hop neighbors at time $t$ as $\cN_{i,t}^{(1)}=\{k|(i,k)\in\cE_t\}$.  For conciseness, denote $\cN_{i,t}=\cN_{i,t}^{(1)}$.  The $k$-hop neighbors at time $t$ are defined as $\cN_{i,t}^{(k)}=\bigcup_{n\in\cN_{i,t}^{(k-1)}}\cN_{n,t}$ for $k\geq 2$.
At time $t$, the node $i$ is $k$-hop away from node $k$ if $k\in\cN_{i,t}^{(k)}$ and $k\notin\cN_{i,t}^{(k-1)}$.

\hl{Remove weights and add discussion on $k$-hop size estimate.  Average degree $d$, and the size $(d-1)d^{k-1}$.}

Next, we define a dynamical system on a time-varying graph $\cG_t$.  Suppose node $i$ has states $x_i\in\cX_i\subset\bR^{n_i}$, and the state dimensions can be different among the nodes.  Denote all states of the graph dynamics
$
    x = [x_1,x_2,\cdots,x_N]\in\cX\subset\bR^{N_x}
$,
where $\cX=\cX_1\times\cX_2\times\cdots\times\cX_N$ and $N_x=\sum_{i=1}^N n_i$.  Furthermore, assume the dynamics at node $i$ is in the following form,
\begin{equation}\label{eqn_nod}
    \dot{x}_i = \alpha_if_i(x_i) + \sum_{j\in\cN_{i,t}^{(k)}} \beta_{ij}f_{ij}(x_i,x_j) \equiv \alpha_if_i(x_i) + F_i(x_i,x,t)
\end{equation}
where the first term accounts for the autonomous dynamics and the summation accounts for the pair-wise interactions among the $k$-hop neighbors; $\alpha_i\in\bR^{n_i\times n_i}$ and $\beta_{ij}\in\bR^{n_i\times n_j}$.  Furthermore, assume that $f_i$ and $f_{ij}$ are Lipschitz and bounded by a unit Lipschitz constant, so that the strength of interaction is determined by the magnitudes of $\alpha_i$ and $\beta_{ij}$.

\hl{Potential concern, need to bound higher-order derivatives too in the truncation process.}

The full-order graph dynamics is denoted compactly as
\begin{equation}
    \dot{x} = f(x) + F(x,x,t)
\end{equation}
where $f=[\alpha_1f_1,\alpha_2f_2,\cdots,\alpha_Nf_N]$ and $F=\diag(F_1,F_2,\cdots,F_N)$.

Furthermore, define a block-diagonal matrix $A$, whose $i$th non-zero block is $\alpha_i$, and a block matrix $B$, whose $ij$th block is $\beta_{ij}$.
Clearly, the nodal interaction is solely due to the non-diagonal terms in $B$.  The sparsity pattern of $B$ is determined by the $k$-hop neighbors, and called the $k$-hop pattern.
The sparsity $s$ of $B$ is defined as
\begin{equation}\label{eqn_dyn}
    s = \frac{1}{N^2}\sum_{i=1}^N \abs{\cN_{i,t}^{(k)}}
\end{equation}
As $k$ increases, $s$ increases and $A$ becomes more dense, which means at least some nodes of the graph interact with more distant nodes.

\begin{rem}
    Conventionally, two nodes are directly connected if the two interact.  But in current definition, two nodes that are $k$-hop apart may still interaction.  We introduce this characteristics to study the impact of distant coupling on the graph dynamics.
\end{rem}

\hl{Still yet to update the examples..., maybe after deciding how we treat the scaling over $k$-hop distance.}

\begin{example}[Kuramoto model]\label{exp:kuramoto}
The governing equation for the Kuramoto model, i.e., networked oscillators, is given by 
\BEA
\dot{x}_i = \omega_i + \sum_{j\in\cN_{i,t}} a_{ij}\sin(x_j-x_i) := F_i(x).
\EEA
In this case, we have $n_i=1$ dimensional variable. The parameters $a_{ij}=a_{ij}(t)> 0$ denote the heterogeneous edge weights $w_{ij,t}$ in previous notation. We will consider the case where the $N\times N$ matrix $(a_{ij})$
is sparse such that it can be rearranged into an almost block diagonal matrix,
\begin{equation}\label{eqn:adj}
    A = \begin{pmatrix} A_{11} & A_{12} & \ldots & A_{1M} \\
    A_{12} & A_{22} & \ldots & A_{2M} \\
    \vdots &  & \ddots & \vdots \\ A_{M1} & A_{M2} & \ldots & A_{MM}
    \end{pmatrix},
\end{equation}

where almost all of the entries of $A_{ij}$ for $i\neq j$ are zero, and $A_{ii} \in \bR^{M_i\times M_i}$ are square matrices. For convenience, we define the nodes in $A_{ii}$ as $\cV_i \subset \cV$, such that $\cup_{i=1}^M \cV_i = \cV$.  

In the subsequence section case, we are interested in predicting the following observable,
$\{z_i, \ldots, z_M\}$, where 
\begin{equation}\label{eqn:obs}
    z_i := \frac{1}{M_i} \sum_{j \in \cV_i} (\cos(x_j),\sin(x_j)), \quad \quad i=1,\ldots, M. 
\end{equation}
{\color{blue} I am not sure how to define $y_i$ in this context.

Let me see if I can understand your notation of Section 3.1. }

For this example, one can indeed choose an observable (or coordinate),
\[
\varphi_i = (\cos(x_i),\sin (x_i))=(y_{1,i},y_{2,i})
\]
and rewrite the Kuramoto system as a closed system of this variable. Specifically, one can write
\BEA
\frac{d}{dt}y_{1,i} &=& \cL^0_i y_{1,i}= F_i \cdot \nabla y_{1,i} = -y_{2,i} \left(\omega_i + \sum_{j=1}^N a_{ij}\left(y_{2,j}y_{1,i}-y_{1,j}y_{2,i})\right)\right),\notag\\
\frac{d}{dt}y_{2,i} &=& \cL^0_i x_{1,i}= F_i \cdot \nabla x_{1,i} = y_{i,i} \left(\omega_i + \sum_{j=1}^N a_{ij}\left(x_{2,j}x_{1,i}-x_{1,j}x_{2,i})\right)\right). \notag
\EEA
In general, such an observable may not exist and we can use the MZ formula directly to expand the dynamical system for the observable. I am not sure Section 3.1 is needed unless if the next example (power system) has such a structure.
\end{example}

\begin{example}[Power system] {\color{blue}I am not sure how to write the power system in the notation above.}
\end{example}

\noindent 

% ----------------------------------
\section{Problem Statement}
% ----------------------------------

Subsequently, the dynamics modeling problem is defined as follows.  
Given observations $z_i\equiv z(t_i)=g(x(t_i))$ and the graph topology $\cG_i=\cG_{t_i}$ over a time sequence $\cT=\{t_1,t_2,\cdots,t_T\}$, evenly sampled with step size $\Dt$, how to predict the future observation $z_{T+1}$ given a new topology $\cG_{T+1}$.  In other words, the goal is to derive a model
\begin{equation}
    z_{T+1} = \hat{f}(z_1,z_2,\cdots,z_T; \cG_1,\cG_2,\cdots,\cG_T, \cG_{T+1})
\end{equation}



==> _arc/_mz.tex <==
Then the dynamics of $\bar{x}$ and $x'$ are
\begin{subequations}\label{eqn_dec}
\begin{align}
    \dot{\bar{x}} &= r^{(1)}(\bar{x}) + r^{(2)}(x) \\
    \dot{x}' &= r^{(3)}(\bar{x}) + r^{(4)}(x)
\end{align}
\end{subequations}
where, define
\begin{subequations}
\begin{align*}
    h^{ij}(\circ) &= \Phi^{i\top}f^j(\circ) \\
    H^{ijk}(\circ,t) &= \Phi^{i\top}F^j(\circ)C(t)\Phi^k
\end{align*}
\end{subequations}
and
\begin{subequations}
\begin{align}
    r^{(1)}(\bx) &= h^{11}(\bx) + H^{111}(\bx,t)\bx \\
    r^{(2)}(x) &= h^{12}(x) + H^{112}(\bx,t) x' + H^{121}(x,t)\bx + H^{122}(x,t)x' \\
    r^{(3)}(\bar{x}) &= h^{21}(\bx) + H^{211}(\bx,t)\bx \\
    r^{(4)}(x) &= h^{22}(x) + H^{212}(\bx,t) x' + H^{221}(x,t)\bx + H^{222}(x,t)x'
\end{align}
\end{subequations}

By definition,
\begin{equation}
    \cP r^{(1),(3)}(\bar{x}) = r^{(1),(3)}(\bar{x}),\quad \cP r^{(2),(4)}(x) = 0.
\end{equation}






Notice that $\cQ\cL\bar{x} = r^{(2)}(x)$,
\begin{align}\nonumber
    N_1(\bx,t) &\equiv \cP\cL\cQ\cL\vz = \cP\cL r^{(2)}(x) \\\nonumber
    &= \left(h^{12}{}'(\bx) + H^{121}{}'(\bx,t)\bx \right) \left(h^{11}(\bx) + H^{111}(\bx,t)\bx \right) \\\label{eqn_mz_i1}
    &+ \left(h^{12}{}'(\bx) + H^{112}(\bx,t) + H^{121}{}'(\bx,t)\bx \right) \left(h^{21}(\bx) + H^{211}(\bx,t)\bx \right)
\end{align}
where $\Box'$ means $\ppf{\Box}{\bx}$.

The multiplications involving $h^{ij}$ and $h^{ij}{}'$ do not change the sparsity pattern since the former is a vector and the latter is block-diagonal.  However, the multiplication between $H^{ijk}$ terms yield a $2k$-hop pattern.  Next, the integral in \eqref{eqn_mz_exp} is
\begin{equation}
    I_1 = \int_0^t \cP e^{(t-s)L} N_1(\bx,t) ds \approx \sum_{i=1}^T w_i N_1(\bx_i,t_i)
\end{equation}
where $w_i$ is appropriately-chosen quadrature weights.  Hence, for each node, the first integral $I_1$ in \eqref{eqn_mz_exp} involves the outputs of $2k$-hop neighbors and the topologies from the past $T$ time steps.



\hl{The following needs to be updated.  Yet, the result becomes very long - two times longer than $N_1$ - so maybe not meaningful to put in the actual equations.  But the conclusion holds: we get $3k$-hop pattern.}


Subsequently, for the second integral $I_2$, some calculations show
\begin{align}\nonumber
    \cP\cL(\cQ\cL)^2\vz &= \left[ \left(\vA^{12}+\vB_2^{112}(\vz,t)+\vB_1^{121}(\vz,t)\right)\left(\vA^{22}+\vB_2^{212}(\vz,t)+\vB_1^{221}(\vz,t)\right) \right. \\\nonumber
    &+ \left(\vB_*^{112}(t)+\vB_*^{121}(t)\right)\left(\vA^{11}\vz+\vB^{111}(\vz,\vz,t)\right) \\
    &+ \left. 2\vB_*^{122}(t)\left(\vA^{21}(\vz)+\vB^{211}(\vz,\vz,t)\right) \right] \left(\vA^{21}+\vB^{211}(\vz,\vz,t)\right)
\end{align}
where multiplications of three $\vB^{ijk}$ terms are involved, indicating a $3k$-hop pattern.



==> _arc/bilinear.tex <==

% ----------------------------------
\subsection{Bilinear Dynamics for Observables}
% ----------------------------------

To facilitate the application of the Mori-Zwanzig formalism to derive the desired model, the input-affine graph dynamics is converted to a bilinear form leveraging the Koopman theory.

For a generic observable $\varphi:\cX_i\mapsto\bC$, the dynamics at node $i$ is
\begin{equation}\label{eqn_kbf}
    \dot{\varphi} = \cL_i^0 \varphi + \sum_{p=1}^{m_i}y_{i,p}\cL_i^p \varphi
\end{equation}
where $\cL_i^p=f_i^p\cdot\nabla_{x_i}$, $p=0,1,\cdots,m_i$, is the Lie derivative associated with $f_i^p$.

\hl{This is probably a strong assumption.  The thought is to derive a bilinear model regardless of the underlying nonlinearity (e.g., linear-cubic for Kuramoto, sin/cos for power grid.)}

For all nodes, $i=1,2,\cdots, N$, suppose there exists a set of observables $\varphi_i:\cX_i\mapsto\bC^{q_i}$, such that
\begin{subequations}\label{eqn_dis}
    \begin{align}
        \cL_i^0\varphi_i &= A_i\varphi_i \\
        \cL_i^p\varphi_i &= B_i^p\varphi_i \\
        x_i &= C_i\varphi_i
    \end{align}
\end{subequations}
where $A_i\in\bC^{q_i\times q_i}$, $B_i^p\in\bC^{q_i\times q_i}$, and $C_i\in\bC^{q_i\times n_i}$.

\hl{If the above holds}

The input at node $i$ is thus
\begin{equation}\label{eqn_yip}
    y_{i,p} = \sum_{j\in\cN_{i,t}^{(k)}} c_{ij,p}(t)^\top x_j = \sum_{j\in\cN_{i,t}^{(k)}} c_{ij,p}(t)^\top C_j\varphi_j \equiv \sum_{j\in\cN_{i,t}^{(k)}} \tilde{c}_{ij,p}(t)^\top \varphi_j
\end{equation}

Applying \eqref{eqn_kbf} to $\varphi_i$ and leveraging \eqref{eqn_dis} and \eqref{eqn_yip}, one obtains,
\begin{equation}
    \dot{\varphi}_i = A_i \varphi_i + \sum_{j\in\cN_{i,t}^{(k)}}\sum_{p=1}^{m_i} (\tilde{c}_{ij,p}(t)^\top \varphi_j)B_i^p \varphi_i
\end{equation}

Denoting the observables of all nodes, $\vtvf=[\varphi_1,\varphi_2,\cdots,\varphi_N]$, the bilinear form of graph dynamics is
\begin{equation}\label{eqn_bln}
    \dot\vtvf = \vA\vtvf + \vB(\vtvf,\vtvf,t)
\end{equation}
where $\vA=\diag(A_1,A_2,\cdots,A_N)$ is block-diagonal, and
\begin{equation}
    \vB(\varphi_i,\varphi_j,t) = \left\{\begin{array}{ll}
        \sum_{p=1}^{m_i} (\tilde{c}_{ij,p}(t)^\top \varphi_j)B_i^p \varphi_i, & j\in\cN_{i,t}^{(k)} \\
        0, & \text{otherwise}
    \end{array}\right.
\end{equation}
Clearly $\vB$ is bilinear in its first two arguments.  Furthermore, note that the sparsity pattern of $\vB$ is determined by the $k$-hop neighbors, and called the $k$-hop pattern.  The sparsity $s$ of $\cB$ is defined as
\begin{equation}
    s = \frac{1}{N^2}\sum_{i=1}^N \abs{\cN_{i,t}^{(k)}}
\end{equation}
As $k$ increases, $s$ increases and $\vB$ becomes more dense, which means at least some nodes of the graph interact with more distant nodes.



% ----------------------------------
\subsection{Coarse-grained Bilinear Dynamics}
% ----------------------------------

At node $i$, suppose $g_i\in\mathrm{span}(\varphi_i)$, and denote $g_i=\Psi_i^{1\hrm}\varphi_i$, where $\Psi_i^1\in\bC^{q_i\times o_i}$.  Define basis $\Phi_i^1 = \Psi_i^1(\Psi_i^{1\hrm}\Psi_i^1)^{-1}$, and choose $\Phi_i^2$ such that $\Psi_i^{1\hrm}\Phi_i^2=O$.  Then,
\begin{equation}
    \varphi_i = \Phi_i^1z_i + \Phi_i^2z_i'
\end{equation}
where $z_i'\in\bC^{q_i-o_i}$ is unresolved variables in the MZ language.

Assembling the bases from all nodes, one obtains,
\begin{equation}
    \vtF^i = \diag[\Phi_1^i, \Phi_2^i,\cdots, \Phi_N^i],\ \vtY^i = \diag[\Psi_1^i, \Psi_2^i,\cdots, \Psi_N^i],\ i=1,2
\end{equation}
where $\vtY^{1\hrm}\vtF^2=O$ and $\vtY^{i\hrm}\vtF^i=I$.  The bases result in a decomposition of resolved and unresolved variables,
\begin{equation}
    \vtvf = \vtF^1 \vz + \vtF^2 \vz'
\end{equation}

Then \eqref{eqn_bln} is decomposed into two equations,
\begin{subequations}\label{eqn_bln_d}
\begin{align}
    \dot{\vz} &= \vtY^{1\hrm}\left[ \vA(\vtF^1\vz + \vtF^2\vz') + \vB(\vtF^1\vz + \vtF^2\vz',\vtF^1\vz + \vtF^2\vz', t) \right] \\
    \dot{\vz}' &= \vtY^{2\hrm}\left[ \vA(\vtF^1\vz + \vtF^2\vz') + \vB(\vtF^1\vz + \vtF^2\vz',\vtF^1\vz + \vtF^2\vz', t) \right]
\end{align}
\end{subequations}

Denote
\begin{equation}
    \vA^{ij} = \vtY^{i\hrm}\vA\vtF^j,\quad \vB^{ijk}(\cdot,\circ,t) = \vtY^{i\hrm}\vB(\vtF^j\cdot,\vtF^k\circ,t)
\end{equation}
Note that since $\vtF$ and $\vtY$ are block-diagonal, $\vA^{ij}$ is still block-diagonal, and the sparsity patterns of $\vB^{ijk}$ are also $k$-hop, same as $\vB$.
For convenience in subsequent derivations, also define,
\begin{equation}
\vB_1^{ijk}(\vz,t) = \ppf{}{\ws}\vB^{ijk}(\ws,\vz,t),\quad 
\vB_2^{ijk}(\vz,t) = \ppf{}{\ws}\vB^{ijk}(\vz,\ws,t),\quad 
\vB_*^{ijk}(t) = \frac{\partial^2}{\partial\ws\partial\vt}\vB^{ijk}(\ws,\vt,t)
\end{equation}

Subsequently \eqref{eqn_bln_d} expands into
\begin{subequations}\label{eqn_bln_xy}
\begin{align}
    \dot{\vz} &= \vr^{(1)}(\vz) + \vr^{(2)}(\vtvf) \\
    \dot{\vz}' &= \vr^{(3)}(\vz) + \vr^{(4)}(\vtvf)
\end{align}
\end{subequations}
where
\begin{subequations}
\begin{align}
    \vr^{(1)}(\vz) &= \vA^{11}\vz + \vB^{111}(\vz,\vz,t) \\\nonumber
    \vr^{(2)}(\vtvf) &= \vA^{12}\vz' + \vB^{112}(\vz,\vz',t) + \vB^{121}(\vz',\vz,t) + \vB^{122}(\vz',\vz',t) \\
    \vr^{(3)}(\vz) &= \vA^{21}\vz + \vB^{211}(\vz,\vz,t) \\\nonumber
    \vr^{(4)}(\vtvf) &= \vA^{22}\vz' + \vB^{212}(\vz,\vz',t) + \vB^{221}(\vz',\vz,t) + \vB^{222}(\vz',\vz',t)
\end{align}
\end{subequations}
